3DMorph: Single-Image-Guided Local 3D Shape Editing and Morphing

Despite recent progress in 3D generation, intuitive editing of existing shapes remains limited. Unlike images, which benefit from well-established inpainting tools, general 3D objects such as meshes still lack simple and effective methods for local shape editing. Existing approaches are often global, domain-specific, require complex user interaction, or focus on appearance (color and texture) rather than geometry. We introduce 3DMorph, a training-free framework for single-image-guided local 3D shape editing and morphing. Given an edited image showing a desired shape modification, our method automatically localizes the relevant 3D region and transfers 2D modifications to 3D while preserving unmodified areas. 3DMorph also enables intermediate shape generation between the original and edited objects, facilitating design exploration. To benchmark editing quality, we introduce Delta3D, an image-guided local 3D editing benchmark with paired ground-truth edits. Experimental results show that 3DMorph translates intuitive 2D edits into 3D, outperforming state-of-the-art generative and editing methods.

==> figures/BB-influence/BB-influence.tex <==



% --- size knobs ---
\newcommand{\panelW}{0.25\textwidth} % width of each subplot
\newcommand{\panelH}{4cm}          % height of each subplot
\newcommand{\panelSep}{30pt}          % horizontal gap between subplots

\begin{figure*}
\begin{tikzpicture}
\begin{groupplot}[
  myaxis,
  width=\panelW,
  height=\panelH,
  group style={group size=3 by 1, horizontal sep=\panelSep},
  tick label style={font=\small},
  label style={font=\small},
  title style={font=\small},
]

% --- (1) CD (down) ---
\nextgroupplot[
  title={$CD\:\downarrow$},
  %ylabel={$CD$},
  ymin=0.020, ymax=0.032,
  grid=both, minor tick num=1, tick align=outside,
  legend pos=north east
]
\addplot[mark=*, color=Morph, thick] coordinates {(all,0.0301) (0.3,0.0263) (0.5,0.0244) (0.7,0.0230) (0.9,0.0217)};
\addplot[mark=o, color=MorphBB, thick] coordinates {(all,0.0230) (0.3,0.0217) (0.5,0.0215) (0.7,0.0207) (0.9,0.0213)};
\legend{3DMorph, 3DMorph-BB}

% --- (2) IoU (%) (up) ---
\nextgroupplot[
  title={$IoU\:(\%)\:\uparrow$},
  %ylabel={IoU (\%)},
  ymin=59, ymax=68,
  grid=both, minor tick num=1, tick align=outside,
  legend pos=south east
]
\addplot[mark=*, color=Morph, thick] coordinates {(all,60.29) (0.3,61.92) (0.5,62.90) (0.7,64.04) (0.9,65.40)};
\addplot[mark=o, color=MorphBB, thick] coordinates {(all,65.17) (0.3,65.98) (0.5,66.04) (0.7,66.64) (0.9,65.56)};
\legend{3DMorph, 3DMorph-BB}

% --- (3) left axis: SAMPLES as bars (shift left) ---
\nextgroupplot[
  title={BB-IoGT + \#Samples},
  ybar,
  bar width=6pt,            % <- keep same on BOTH axes
  enlarge x limits=0.18,     % <- same padding on BOTH axes
  ymin=0, ymax=900,
    ymajorgrids,                % <--- add horizontal grid lines
    grid style={dashed,gray!50}, % <--- style of the grid
  legend pos=north west
]
\addplot+[fill=gray, draw=gray, bar shift=-6pt] coordinates {
  (all,816)
  (0.3,650)
  (0.5,527)
  (0.7,306)
  (0.9,132)
};
\addlegendentry{Samples}

\end{groupplot} % <--- close the group BEFORE overlaying

% --- Overlay RIGHT y for panel (c3r1): BB-IoGT as bars (shift right) ---
\begin{axis}[
  myaxis,
  width=\panelW,
  height=\panelH,
  at={(group c3r1.center)}, anchor=center,
  axis y line*=right,
  axis x line=none,
  ybar,
  bar width=6pt,            % <- SAME as above
  enlarge x limits=0.18,     % <- SAME as above
  yticklabel style={color=orange},
  y label style={color=orange},
  %ylabel={BB-IoGT},
  ymin=0, ymax=1.0,          % bars should start at 0 for bar charts
  trim axis left, trim axis right,
  clip=false,
    ymajorgrids,                % <--- add horizontal grid lines
    grid style={dashed,orange!50} % <--- style of the grid
]
\addplot+[fill=orange, draw=orange, bar shift=+6pt, fill opacity=0.45] coordinates {
  (all,0.5717)
  (0.3,0.688)
  (0.5,0.7574)
  (0.7,0.8817)
  (0.9,0.991)
};
\addlegendentry{BB-IoGT}
\end{axis}




\end{tikzpicture}
\caption{Influence of the bounding box. TOOD.}
\label{fig:BB-influence}
\end{figure*}





%%%%%%
% \begin{figure*}
% \centering

% % First plot
% \begin{minipage}{0.33\textwidth}
% \begin{tikzpicture}
% \begin{axis}[
%     axis lines=left,
%     xlabel={Threshold},
%     title={$CD\:\downarrow$},
%     ylabel= {$CD$},
%     xtick={0,1,2,3,4},
%     xticklabels={all, 0.3, 0.5, 0.7, 0.9},
%     ymin=0.02, ymax=0.032,
%     grid=major,
%     width=\textwidth, height=5cm
% ]
% \addplot[mark=*, color=cyan, thick] coordinates {
%     (0,0.0301)
%     (1,0.0263)
%     (2,0.0244)
%     (3,0.023)
%     (4,0.0217)
% };
% \addplot[mark=o, color=blue, thick] coordinates {
%     (0,0.023)
%     (1,0.0217)
%     (2,0.0215)
%     (3,0.0207)
%     (4,0.0213)
% };
% \end{axis}
% \end{tikzpicture}
% \end{minipage}
% \hfill
% % First plot
% \begin{minipage}{0.33\textwidth}
% \begin{tikzpicture}
% \begin{axis}[
%     axis lines=left,
%     xlabel={Threshold},
%     title={$IoU\:(\%)\:\uparrow$},
%     ylabel= {$IoU$},
%     xtick={0,1,2,3,4},
%     xticklabels={all, 0.3, 0.5, 0.7, 0.9},
%     ymin=59, ymax=68,
%     grid=major,
%     width=\textwidth, height=5cm
% ]
% \addplot[mark=*, color=cyan, thick] coordinates {
%     (0,60.29)
%     (1,61.919999999999995)
%     (2,62.9)
%     (3,64.03999999999999)
%     (4,65.4)
% };
% \addplot[mark=o, color=blue, thick] coordinates {
%     (0,65.16999999999999)
%     (1,65.98)
%     (2,66.03999999999999)
%     (3,66.64)
%     (4,65.56)
% };
% \end{axis}
% \end{tikzpicture}
% \end{minipage}
% \hfill
% % third plot
% \begin{minipage}{0.33\textwidth}
% \begin{tikzpicture}
% % LEFT Y-AXIS: absolute counts (130–820)
% \begin{axis}[
%   axis y line*=left,
%   axis x line*=bottom,
%   xlabel={Threshold},
%   ylabel={\# Samples},
%   y label style={color=black},
%   yticklabel style={color=black},
%   ymin=130, ymax=820,
%   xtick={0,1,2,3,4},
%   xticklabels={all, 0.3, 0.5, 0.7, 0.9},
%   grid=major,
%   width=\textwidth, height=5cm,
%   legend style={draw=none, at={(0.02,0.98)}, anchor=north west}
% ]
% % <-- replace this series with your real counts
% \addplot[mark=square*, thick] coordinates {(0,130) (1,260) (2,410) (3,620) (4,820)};
% \addlegendentry{Samples (left y-axis)}
% \end{axis}

% % RIGHT Y-AXIS: metric in [0,1]
% \begin{axis}[
%   axis y line*=right,
%   axis x line=none, % share x-axis from the first axis
%   ylabel={IoU},
%   y label style={color=blue},
%   yticklabel style={color=blue},
%   ymin=0, ymax=1,
%   width=\textwidth, height=5cm
% ]
% % your metric series in 0–1
% \addplot[mark=*, color=blue, thick] coordinates {
%   (0,0.6029) (1,0.6192) (2,0.629) (3,0.6404) (4,0.654)
% };
% \end{axis}

% \end{tikzpicture}
% \end{minipage}

% \end{figure*}


%%%%%%%%

% \begin{tikzpicture}
% \begin{axis}[
%     axis lines=left,
%     xlabel={Threshold},
%     ylabel={IoU},
%     xtick={0,1,2,3,4},
%     xticklabels={all, 0.3, 0.5, 0.7, 0.9},
%     ymin=0.55, ymax=0.7,
%     grid=major,
%     width=0.5\textwidth, height=6cm
% ]

% % Your new data
% \addplot[
%     mark=*,
%     color=cyan,
%     thick
% ] coordinates {
%     (0,0.6029)
%     (1,0.6192)
%     (2,0.629)
%     (3,0.6404)
%     (4,0.654)
% };
% \addplot[
%     mark=o,
%     color=blue,
%     thick
% ] coordinates {
%     (0,0.6517)
%     (1,0.6598)
%     (2,0.6604)
%     (3,0.6664)
%     (4,0.6556)
% };


% \end{axis}
% \end{tikzpicture}


==> figures/morphing/morph-fig.tex <==
\def\imagewidth{0.15}

\begin{figure*}[!t]
\centering
\begin{tabular}{cccccc}
\toprule
\centering  $O=\mathcal{O}_0$ &  $\mathcal{O}_{\frac{1}{5}M}$ &  $\mathcal{O}_{\frac{2}{5}M}$ &  $\mathcal{O}_{\frac{3}{5}M}$ &  $\mathcal{O}_{\frac{4}{5}M}$ &  $\tilde{O}=\mathcal{O}_M$  \\ 
\midrule
\raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_00.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_03.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_07.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_11.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_15.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/bike/bike_-15_-30_20.png}} \\
\midrule
\raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_00.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_05.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_10.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_15.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_20.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/coffee/coffee_-35_-19_25.png}} \\
\midrule
\raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_00.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_03.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_07.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_11.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_15.png}}
& \raisebox{-0.5\height}{\includegraphics[width=\imagewidth\textwidth]{images/morphing/car/car_225_-20_20.png}} \\
\bottomrule
\end{tabular}
\caption{Morphing results. The left and right columns show the original and edited objects, respectively, while the four middle columns display intermediate shapes at increasing morph steps.}
\label{fig:morphing}
\end{figure*} 

% Morphing results. The left and right columns show the original and edited objects, respectively, while the four columns in between display intermediate shapes at increasing morph steps.
